DTL: Data Tumbling Layer. A Composable Unlinkability for Smart Contracts

We propose Data Tumbling Layer (DTL), a cryptographic scheme for non-interactive data tumbling. The core concept is to enable users to commit to specific data and subsequently re-use to the encrypted version of these data across different applications while removing the link to the previous data commit action. We define the following security and privacy notions for DTL: (i) no one-more redemption: a malicious user cannot redeem and use the same data more than the number of times they have committed the data; (ii) theft prevention: a malicious user cannot use data that has not been committed by them; (iii) non-slanderabilty: a malicious user cannot prevent an honest user from using their previously committed data; and (iv) unlinkability: a malicious user cannot link tainted data from an honest user to the corresponding data after it has been tumbled. To showcase the practicality of DTL, we use DTL to realize applications for (a) unlinkable fixed-amount payments; (b) unlinkable and confidential payments for variable amounts; (c) unlinkable weighted voting protocol. Finally, we implemented and evaluated all the proposed applications. For the unlinkable and confidential payment application, a user can initiate such a transaction in less than $1.5$s on a personal laptop. In terms of on-chain verification, the gas cost is less than $1.8$ million.

==> acro.tex <==
\usepackage{acro}
\acsetup{single}


\DeclareAcronym{VC}{
  short = VC,
  long  = Verifiable Computation ,
}
\newcommand{\systemvc}{\ac{VC}\xspace}

\DeclareAcronym{MPB}{
  short = MPB,
  long  = Merkle Pyramid Builder ,
}
\newcommand{\system}{\ac{MPB}\xspace}


\DeclareAcronym{PoS}{
  short = PoS,
  long  = Proof-of-Stake,
}
\newcommand{\PoS}{\ac{PoS}\xspace}

\DeclareAcronym{PoW}{
  short = PoW,
  long  = Proof-of-Work,
}
\newcommand{\PoW}{\ac{PoW}\xspace}

\DeclareAcronym{DoS}{
  short = DoS,
  long  = Denial of Service,
}
\newcommand{\DoS}{\ac{DoS}\xspace}

\DeclareAcronym{DDoS}{
  short = DDoS,
  long  = Distributed Denial-of-Service,
}
\newcommand{\DDoS}{\ac{DDoS}\xspace}

\DeclareAcronym{ENS}{
  short = ENS,
  long  = Ethereum Name Service,
}
\newcommand{\ENS}{\ac{ENS}\xspace}


\DeclareAcronym{TC}{
  short = TC,
  long  = Tornado Cash,
}
\newcommand{\TC}{\ac{TC}\xspace}


\DeclareAcronym{ASS}{
  short = ASS,
  long  = anonymity set size,
}
\newcommand{\ASS}{\ac{ASS}\xspace}

\DeclareAcronym{TN}{
  short = TN,
  long  = Typhoon Network,
}
\newcommand{\TN}{\ac{TN}\xspace}


\DeclareAcronym{TP}{
  short = TP,
  long  = Typhoon Cash,
}
\newcommand{\TP}{\ac{TP}\xspace}



\DeclareAcronym{DeFi}{
  short = DeFi,
  long  = Decentralized Finance,
}
\newcommand{\DeFi}{\ac{DeFi}\xspace}


\DeclareAcronym{ZKP}{
  short = ZKP,
  long  = Zero-knowledge proof,
}
\newcommand{\ZKP}{\ac{ZKP}\xspace}


\DeclareAcronym{CEX}{
  short = CEX,
  long  = Centralized Exchange,
}
\newcommand{\CEX}{\ac{CEX}\xspace}
\newcommand{\CEXes}{\acp{CEX}\xspace}


\DeclareAcronym{DEX}{
  short = DEX,
  long  = Decentralized Exchange,
}
\newcommand{\DEX}{\ac{DEX}\xspace}
\newcommand{\DEXes}{\acp{DEX}\xspace}

\DeclareAcronym{CLI}{
  short = CLI,
  long  = command line interface,
}
\newcommand{\CLI}{\ac{CLI}\xspace}

\DeclareAcronym{TEE}{
  short = TEE,
  long  = Trusted Execution Environment,
}
\newcommand{\TEE}{\ac{TEE}\xspace}

\DeclareAcronym{P2P}{
  short = P2P,
  long  = peer-to-peer,
}
\newcommand{\PtP}{\ac{P2P}\xspace}

\DeclareAcronym{APY}{
  short = APY,
  long  = annual percentage yield,
}
\newcommand{\APY}{\ac{APY}\xspace}


\DeclareAcronym{DApp}{
  short = DApp,
  long  = Decentralized Application,
}
\newcommand{\DApp}{\ac{DApp}\xspace}
\newcommand{\DApps}{\acp{DApp}\xspace}

\DeclareAcronym{CeFi}{
  short = CeFi,
  long  = Centralized Finance,
}
\newcommand{\CeFi}{\ac{CeFi}\xspace}

\DeclareAcronym{MEV}{
  short = MEV,
  long  = Miner Extractable Value,
}
\newcommand{\MEV}{\ac{MEV}\xspace}

\DeclareAcronym{EV}{
  short = EV,
  long  = Extractable Value,
}
\newcommand{\EV}{\ac{EV}\xspace}

\DeclareAcronym{BEV}{
  short = BEV,
  long  = Blockchain Extractable Value,
}
\newcommand{\BEV}{\ac{BEV}\xspace}

\DeclareAcronym{TVL}{
  short = TVL,
  long  = total value locked,
}
\newcommand{\TVL}{\ac{TVL}\xspace}


\DeclareAcronym{AMM}{
  short = AMM,
  long  = Automated Market Maker,
}
\newcommand{\AMM}{\ac{AMM}\xspace}
\newcommand{\AMMs}{\acp{AMM}\xspace}

\DeclareAcronym{FaaS}{
  short = FaaS,
  long  = Front-running as a Service,
}
\newcommand{\FaaS}{\ac{FaaS}\xspace}
\newcommand{\FaaSs}{\acp{FaaS}\xspace}

\DeclareAcronym{HFT}{
  short = HFT,
  long  = High-frequency Trading,
}
\newcommand{\HFT}{\ac{HFT}\xspace}


\DeclareAcronym{PBS}{
  short = PBS,
  long  = Proposer-Builder Separation,
}
\newcommand{\PBS}{\ac{PBS}\xspace}

\DeclareAcronym{OFAC}{
  short = OFAC,
  long  = Office of Foreign Assets Control ,
}
\newcommand{\OFAC}{\ac{OFAC}\xspace}


\DeclareAcronym{PGA}{
  short = PGA,
  long  = Priority Gas Auction,
}
\newcommand{\PGA}{\ac{PGA}\xspace}
\newcommand{\PGAs}{\acp{PGA}\xspace}

\DeclareAcronym{BRF}{
  short = BRF,
  long  = Back-run Flooding,
}
\newcommand{\BRF}{\ac{BRF}\xspace}

\DeclareAcronym{FRF}{
  short = FRF,
  long  = Front-run Flooding,
}
\newcommand{\FRF}{\ac{FRF}\xspace}

\DeclareAcronym{PRG}{
  short = PRG,
  long  = Priority Gas Auction,
}
\newcommand{\PRG}{\ac{PRG}\xspace}

%% design patterns
\DeclareAcronym{AE}{
  short = AE,
  long  = Atomic Execution,
}
\newcommand{\AEE}{\ac{AE}\xspace}


\DeclareAcronym{BEET}{
  short = BEET,
  long  = Break-even Extraction Threshold,
}
\newcommand{\BEET}{\ac{BEET}\xspace}


\DeclareAcronym{BAD}{
  short = BAD,
  long  = Breaking Atomicity and Determinism,
}
\newcommand{\BAD}{\ac{BAD}\xspace}

%% novel design

\DeclareAcronym{AM}{
  short = AM,
  long  = anonymity mining,
}
\newcommand{\AM}{\ac{AM}\xspace}


\DeclareAcronym{dfmm}{
  short = DFMM,
  long  = Dynamic Fee Market Maker,
}
\newcommand{\dfmm}{\ac{dfmm}\xspace}

\DeclareAcronym{dfaamm}{
  short = A$^2_F$MM,
  long  = Automated Arbitrage and Fee Market Maker,
}
\newcommand{\dfaamm}{\ac{dfaamm}\xspace}


\DeclareAcronym{MVI}{
  short = MVI,
  long  = Minimum Victim Input,
}
\newcommand{\MVI}{\ac{MVI}\xspace}


\DeclareAcronym{BSC}{
  short = BSC,
  long  = Binance Smart Chain,
}
\newcommand{\BSChain}{\ac{BSC}\xspace}

\DeclareAcronym{ETH}{
  short = ETH,
  long  = Ethereum,
}
\newcommand{\ETHchain}{\ac{ETH}\xspace}





==> short-prelim.tex <==
% !TEX root = main-formalism.tex
\section{Preliminaries}
\label{sec:prelim}

% \todo{We can move the definitions in this section to the appendix if we need space (and only put the API if needed)}

% \subsection{Cryptographic Primitives}
\paragraph{Notation}
We denote the security parameter by $\sparam$ and a negligible function in $\sparam$ by 
$\mathtt{negl}(\lambda)$.
% We express a pair of public and private keys by $(\pk, \sk)$.
% Moreover, we require that $\pk$ can always be efficiently derived from $\sk$, 
% and we denote $\fun{extractPK}(\sk)=\pk$ to be the deterministic function to derive $\pk$ from $\sk$. 
%$k||r$ denotes concatenation of two binary string $k$ and $r$. 
We let $[n]$ denote the set $\{1,\dots, n\}$.
We use $(x_i)_{i=1}^{n}$ to denote a list of $n$ elements, $(x_1, \dots, x_n)$.
%We denote $\mathbb{Z}_{\geq a}$ to denote the set of integers that are
%greater or equal $a$, $\set{a, a+1, \dots}$. 
We let PPT denote probabilistic polynomial time.
%We use a shaded area \gamechange{$i,j,k$} to denote 
%the private inputs in the relation $\statement : \{ (a,b,c; \pInput{i, j, k}): f(a,b,c,\pInput{i, j, k}) =\true\}$.
%We use $\statement[a,b,c \dots]$ to denote those fixed and public values of an instance of the relation $\statement$.
% We denote by $\FF$ a cyclic group of prime order $\primeorder$ and 
% by $\generator$, we denote a fixed generator of such group. 
% Let $\mathcal G$ be polynomial time algorithm that on input $\sparam$, outputs
% $(p,g,\FF)$.
We define the security properties of our protocol as games written in pseudocode.
These games invoke a probabilistic-polynomial time (PPT) adversary, \adv, with
access to some oracles. 

% We use letters $\alice$ to  $\zoe$ to identify clients in a protocol. 
% Finally, we consider two hash functions: (i) $\hashs$ takes as input 
% a bitstring and outputs a scalar (i.e., $\hashs: \{0,1\}^* \to \mathbb{Z}_q$); (ii) $\hashp$ 
% takes as input a bitstring and outputs 
% an element of $\FF$ (i.e., $\hashp: \{0,1\}^* \to \FF$).

% \added[id=todo]{May modified this part to ZKSnark if only ZKSnark is used}
\iffalse
\pparagraph{Noninteractive Zero-knowledge Proofs (NIZK)}  
Zero Knowledge Proof (ZKP)
is a cryptographic primitive that allows a prover to convince the verifier about
the correctness of some assertions without providing any meaningful information
to the verifier. Several ZKPs require multiple rounds of interactions between
prover and verifier.  

NIZK is, on the other hand, one of the variants of ZKP in which there is no
need for interaction between the verifier and prover. As shown
in~\cite{blum-stoc88:NIZK}, NIZK can be realized if there is a shared common
reference string between verifier and prover.  Adapting the definition
from~\cite{ars-bootle15,zether-bunz-2020}, we define NIZK as follows. 
\begin{definition}
a \textit{non-interactive zero-knowledge proof} (NIZK) system consists of 3
algorithm $(\fun{NIZK.Setup},$ $\fun{NIZK.Prove},$ $\fun{NIZK.Verify})$ relative to
a relation $R$ defining the language $\mathcal L_R := \{\statement~|~\exists w: (\statement, w)
\in R\}$ where $\statement$ is that statement and $w$ is a witness, such that:
\begin{itemize}
    \item $\mathsf{crs} \leftarrow $\fun{NIZK.Setup}($\sparam$) takes as input
        the security parameter, and outputs the common reference string
        $\mathsf{crs}$
    \item $\pi \leftarrow $\fun{NIZK.Prove}($\mathsf{crs}, \statement, w$) takes as
        input the reference string $\mathsf{crs}$, any $(s,w)\in R$ , outputs a
        proof $\pi$ that $(s,w) \in R$.
    \item $0/1 \leftarrow $\fun{NIZK.Verify}($\mathsf{crs},\statement, \pi$) takes as
        input the reference string $\mathsf{crs}$, a statement $s$, and proof
        $\pi$, output $1$ iff the proof $\pi$ verifies that $s\in \mathcal
        L_R$, otherwise, return $0$
\end{itemize}
A Zero-knowledge proof $\pi$ for the relation $R$:
  $$R:\set{(a,b,c, \dots;{x, y, z \dots}): f(a,b,c, \dots;x,y,z \dots)}$$
means that prover has a knowledge of $(x,y,z, \dots)$ such that $f(a,b,c, \dots;x,y,z \dots)$
is true, where $a,b,c \dots$ are public variables. 
% We use $\statement[a,b,c \dots]$ to denote an instance of the statement where $a,b,c\dots$ 
% has fixed values.
\end{definition}
{This work uses NIZK proof system that achieves \emph{zero-knowledge, soundness,} and \emph{completeness}. 
We defer the formal definitions to~\cite{nizk-oded-1991}}.
\fi

{
\iffalse
\pparagraph{Collision-Resistant Hash Functions} 
A family $H$ of hash functions is collision-resistant, 
iff for all PPT $\mathcal A$ given $h\sample H$, the probability that $\mathcal{A}$ finds $x, x'$, such that
$h(x)=h(x')$ is negligible.
We refer to the cryptographic hash function $h$ as a fixed function, $h:
\bset^* \to \bset^\lambda$. For the formal definitions of the cryptographic
hash function family, we refer the reader to~\cite{rogaway2004cryptographic}.
\fi

\iffalse
\pparagraph{Random Oracle}
We model all hash functions in the random oracle model. Any user can query a hash function
$h$ that takes as input a bit string $x\in \bset^*$ and returns a uniformly random string from $\bset^{\lambda}$, where $\lambda$ is the security parameter.
Also, upon repeated queries, $h$ \emph{deterministically} outputs the same answer.
\fi

\pparagraph{\zksnark}
A zero-knowledge Succinct Non-interactive ARgument of Knowledge
(\zksnark) is a ``succinct'' non-interactive zero-knowledge proofs (NIZK) for arithmetic circuit satisfiability. 
For a field $\FF$, an arithmetic circuit $C$ takes
as inputs elements in $\FF$ and outputs elements in $\FF$. 
We adopt a similar definition from Zerocash~\cite{sasson2014zerocash}
to define the arithmetic circuit satisfiability problem.
An arithmetic circuit satisfiability problem of a circuit ${C}:\FF^n\times\FF^h\rightarrow \FF^l$
is captured by the relation $R_C=\set{(\statement,\witness)\in \FF^n\times \FF^h: C(x,\witness) = 0^l}$, with 
the language $\mathcal L_C = \set{\statement \in \FF^n~|~\exists~\witness \in \FF^h~s.t~C(\statement,\witness) = 0^l}$. 

% \todo{Should we also add the "large bracket" notation we are using later for the zero knowledge proofs?}
%\todo{We use "C" for both circuits and contracts, which is confusing. Maybe replace "C" with "$\Pi$" for proofs?


%@Duc says: I changed the font and i change to relation R when i describe the circuit check the construction,   $Pi$ is zkproof itself
%}

\begin{definition}[\zksnark~\cite{groth2016size}]
\label{def:zksnarks}
\zksnark, $\Pi$, for arithmetic circuit satisfiability is a triple of 
algorithms $(\mathtt{Setup}, \mathtt{Prove}, \mathtt{Verify})$: 
\begin{itemize}[leftmargin=0.5cm]
    \item $(\pk, \vk) \leftarrow \fun{Setup}(\sparam, C)$ 
    takes as input the security parameter and the arithmetic circuit $C$, outputs
    a proving key $\pk$, and a verification key $\vk$. The public parameters, $\pp$, is given implicitly
    to both proving and verifying algorithms.
    \item $\pi\leftarrow \fun{Prove}(\pk,\statement,\witness)$ takes as input the
    evaluation key $\ek$ and $(x, \witness) \in R_C$, outputs a proof 
    $\pi$ for the statement $x \in \mathcal{L}_C$
    \item $0/1\leftarrow\fun{Verify}(\vk, \statement, \pi)$ takes as input the verification
    key $\vk$, the public input $x$, the proof $\pi$,  outputs $1$ if $\pi$ is valid proof
    for  $x \in \mathcal{L}_C$. 
\end{itemize}
\end{definition}

Apart from \emph{correctness, soundness,} and \emph{zero-knowledge} properties, 
a \zksnark requires two additional properties, \textit{succinctness} and 
{\textit{simulation extractability}}.



% \pparagraph{Collision resistant hash function}
% \label{hash_function} We denote $H$ to be a family of collision resistant hash functions, if for any PPT $\mathcal A$ given $h\sample H$, the probability that $\mathcal{A}$ learns $x, x'$, such that $h(x)=h(x')$ is negligible. The cryptographic hash function $h$ is referred to as the fixed function $h: \bset^* \to \bset^\lambda$. 



\pparagraph{Commitment Scheme} 
A commitment scheme contains two operations: committing and revealing. During the committing operation, a user commits to selected values while concealing them from others. The user can choose to reveal the committed value during the revealing operation.  
\begin{definition}[Commitment Scheme]
\label{def:commitscheme}
  A commitment scheme, $\commit$ defined over $(\mathcal{X}, \mathcal{Y})$,
  consists of two algorithms: 
 \begin{itemize}[leftmargin=0.5cm]
      \item $\pp_{\mathsf{commit}} \leftarrow \fun{Setup}(\sparam)$ takes as
          input the security parameter, $\sparam$, it outputs the public
          parameters are implicit input to all subsequent algorithms.
      \item $\cm \leftarrow \fun{Commit}(m; r)$ accepts a message $m$ and a
          secret randomness $r$ as inputs and returns the commitment string
          $\cm$. 
      \item $0/1 \leftarrow \fun{Verify}(m, \cm; r)$ accepts a message $m$, a
          commitment $\cm$ and a value $r$ as inputs, and returns $1$ if the
          commitment is opened correctly and $0$ otherwise.
  \end{itemize}
\end{definition}
\noindent A commitment scheme should satisfy two security requirements:
(i) \emph{Binding:} Except for a negligible probability, no
probabilistic-polynomial time adversary can
efficiently produce $\cm$, $(m_1, r_1)$ and $(m_2, r_2)$ such that
$\fun{Verify}(m_1, \cm; r_1) = \fun{Verify}(m_2, \cm; r_2) = 1$ and $m_1 \neq
m_2$,
(ii) \emph{Hiding:} Except for a negligible probability, $\cm$ does not reveal
anything about the committed data.
{We can instantiate $\com$ with a hash function $h$ in the random oracle model.}

% \todo{Maybe we don't need ADS or at least the definition of ADS here}

% \todo{vector commitment/authenticated data structure}
\pparagraph{Merkle Tree}~\label{pp:merkle-tree}
% An authenticated data structure (ADS) is suitable for particular operations
% that any verifier can perform.
% The verifier can then efficiently verify the validity of the proof results.
% This is achieved by the prover generating a concise proof that the verifier can
% verify using the outcome of each operation. 
In this work, we focus solely on the Merkle tree, which is an authenticated data structure used for set membership.
% We are solely interested in a data structure for set membership in this work.
% \begin{definition}[Authenticated Data Structure]
%   \label{def:ADS}
%   An authenticated data structure consists of four algorithms $\Pi=(\initialize,$ $\fun{Prove},$ $\fun{Verify},$ $\fun{Update})$.
%  \begin{itemize}[leftmargin=0.5cm]
%     \item $y\leftarrow\initialize(\sparam, X)$ takes the security parameter and a list $X=(x_1,\dots, x_n)$ as inputs and outputs $y \in \bset^\lambda$.
%     \item $\pi \leftarrow \prove(i, x, X)$ takes an element $x\in \bset^*, 1\leq i \leq n$ and a $X = (x_1, \dots, x_n)$ as inputs, and outputs the proof that $x=x_i \in X$.
%     \item $0/1\leftarrow \mkverify(i, x, y, \pi)$ takes an element $x_i \in \bset^*, 1 \leq i \leq n, y\in \bset^\lambda$ and a proof $\pi$ as inputs. 
%     It outputs $1$ if $x = x_i$ and $y=\initialize(\sparam, X)$ and $0$ otherwise.
%     \item $y' \leftarrow \update(i,x,X)$ takes an element $x \in \bset^*, 1 \leq i \leq n$ and $X$ as inputs, and outputs $y' = \initialize(\sparam, X')$ where $X'$ is $X$ but $x_i \in X$ is replaced by $x$.
%   \end{itemize}
% \end{definition}
% or RSA-accumulator~\cite{benaloh1993one,boneh2019batching} are examples of authenticated data structures.
A Merkle tree leverages a collision-resistant hash function to construct
the data structure. A Merkle tree consists of four algorithms that work as
follows:

\begin{definition}[Merkle Tree]
\label{def:ads}
A Merkle tree, $\mathsf{MT}$ defined over $(\mathcal{X}^n, \mathcal{Y})$, consists of the following algorithms: 
\begin{itemize}[leftmargin=0.5cm]
     \item $\rt\leftarrow\initialize(\sparam, \seqx)$ takes the security parameter and
         a list $\seqx$ as inputs, where $x_i \in \mathcal{X}$, $n$ is a power of $2$, and
         the algorithm outputs $\rt \in \mathcal{Y}$.

     \item $\adsproof \leftarrow \prove(j, x, \seqx)$ takes an element $x$, an
         index,  $j\in [n]$, and a sequence $\seqx$ as inputs, and outputs the
         proof $\pi$, which can prove that $x$ is the $j^{th}$ element in the
         sequence $\seqx$. 
    
    \item $0/1\leftarrow \mkverify(j, x, \rt, \adsproof)$ takes an index $j \in [n]$,
        an element $x$, a root, $\rt\in \bset^\lambda$ and a proof $\adsproof$ as
        inputs. The algorithm outputs $1$ if $x$ is the $j^{th}$ element in
        \seqx and $0$ otherwise.

%    \item $\rt' \leftarrow \update(j,x,\seqx)$ takes an element $x$, an index $
%        j \in [n]$ and a sequence $\seqx$ as inputs, and outputs $\rt' =
%        \initialize(\sparam, \seqx)$ where $x_j \in \seqx$ is replaced with
%        $x$. 
  \end{itemize}

\end{definition}

%   \noindent\emph{Efficient Merkle tree update.} 
%   If the internal structure of the Merkle tree is stored, 
%   % the entire hash tree will need to be recalculated from scratch~\cite{boneh2020graduate}. 
%   the computational cost of updating a Merkle hash tree is $O(\log n)$. This
%   can be done by modifying at most $O(\log n)$ internal nodes of the tree. 

   A Merkle tree should satisfy \emph{correctness} and \emph{security}. 
   For the formal
   definitions of these properties, we refer to the cryptography introduction
   book of Boneh and Shoup~\cite{boneh2020graduate}. 
   % \tre
   % {We can instantiate $\tree$ with a collision-resistant hash function.}
   
% \iffalse
\pparagraph{Tagging Scheme} In this work, we use the definition of the tagging
scheme from~\cite{lai2019omniring}. However, our tagging scheme does not
require the homomorphic property as defined in their protocol. Hence, we
modified the security experiments to not use the related input oracles. 

%\zhiyong{It seems to me the one-wayness and the pseudorandomness are almost exactly the binding and hiding properties of a commitment scheme, respectively.}
%{\comment[id=duc]{using this definition may avoid talking about commitment and hashing explicitly.}}
A tagging scheme, $\mathsf{TAG}$ defined over $(\mathcal{K}, \mathcal{P}, \mathcal{T})$, is a
triple of algorithms, where: 
\begin{itemize}[leftmargin=0.5cm]
    \item $\tagpp\gets \tagsetup(\sparam)$: On input the
        security parameter $\sparam$, it outputs the public parameter,
        $\tagpp$. The public parameters are implicitly input to all
        subsequent algorithms. 
    \item $\dcmcoinpk \leftarrow \tagkeygen(\dcmcoinsk)$: On input the key
        $\dcmcoinsk$ from the secret key space~$\mathcal{K}$, it \emph{deterministically} outputs a public key
        $\dcmcoinpk \in \mathcal{P}$.
    \item $\key{tag} \leftarrow \tageval(\dcmcoinsk)$: On input the secret
        key $\dcmcoinsk$, it \emph{deterministically} outputs the tag  $\key{tag} \in \mathcal{T}$. 
\end{itemize}
The tagging scheme should satisfy \emph{one-wayness}, \emph{collision-resistance}, and \emph{pseudo-randomness}. 
% \fi

\pparagraph{Encryption Scheme} For arbitrary data construction, we need to use encryption scheme defined as follows. 
\begin{definition}
A public-key encryption scheme,
$\mathtt{E}$, defined over $(\mathcal{M}, \mathcal{C})$, works as follows: 
\begin{itemize}[leftmargin=0.5cm]
    \item  $(\dk, \ek) \leftarrow \fun{KGen}(\sparam)$: On input the security
        parameter $1^\lambda$, the algorithm outputs a pair of decryption
        and encryption keys, $(\dk, \ek)$. 
    \item  $c \leftarrow \fun{Enc}(\ek, m; r)$: On input an encryption key, \ek,
    a message, $m \in \mathcal{M}$, and randomness $r$, the algorithm outputs a ciphertext, $c \in \mathcal{C}$. 
    \item  $m \leftarrow \fun{Dec}(\dk, c)$: On input a decryption key, $\dk$
    and a ciphertext $c \in \mathcal{C}$, the algorithm outputs a message, $m\in \mathcal{M}$.
\end{itemize}
\end{definition}
The encryption scheme $\mathtt{E}$ should be correct and satisfy ciphertext
indistinguishability under chosen-plaintext attacks (IND-CPA). For some applications, 
we require the encryption scheme to be \emph{additively homomorphic}. 
We assume there is a deterministic function $\fun{derive}$, which takes as input
the decryption key and outputs the encryption key, i.e. $\ek = \fun{derive}(\dk)$. 

 
% \iffalse

% \iffalse
% \comment[id=pedro]{Somme comments here:\\
%  - We might want to use terms other than $\dcmcoinsk$ and $\dcmcoinpk$ here, since the tagging scheme is independent of the DCM scheme.\\
%  - I would explicitly mention that the tagging scheme we are considering here is that of~\cite{lai2019omniring} but without the ``homomorphic'' or the ``related-input'' part.\\
%  - During the last discussion, we thought that OneWay and MultiTag are equivalent. If so, I would make it explicit here (e.g., stating it in a lemma). }
% \fi


% \fi
% \todo{Can we prove pseudorandomness purely from hash or the function for
% nullifier to be a prf? ? can oneway reduce to hiding of commitment scheme? We
% need something weaker than collision-resistance must be defined here. Attempted
% to define one, but it seems equivalent for a PPT $\mathcal{A}$}

\iffalse
\comment[id=zhiyong]{I want to add the definition here because later in the swap, one may want to prove he knows $x$ such that $y=g^x$. This coincides with the keys in the Elgamal Encryption scheme, so we can avoid introducing another key pair.}
\todo{@zhiyong: do we need to specify elgama?}
\begin{definition}[Elgamal Encryption]
    We make extensive use of confidential assets in our applications of \DDM. For ease of elaboration, we assume the Elgamal Encryption scheme $\mathcal{E}$ will be used, which is defined by the following algorithms:
   \begin{itemize}[leftmargin=0.5cm]
        \item $\encpp \gets \encsetup(\sparam) $. On inputting the security parameter, generate a cyclic group $G$, and agree on the generator $g$. Output $\encpp$ as $(G, g)$.
        \item $(\sk, \pk) \gets \enckeygen(\encpp)$. Randomly sample $\sk \gets G$, and compute $\pk\gets g^\sk$.
        \item $c \gets \encrypt(m, \encpp, \pk)$. Encrypt the message $m$ as $c=(c_1, c_2)=(g^r, g^m \pk^r)$ for some randomly sampled $r\gets G$.
        \item $m \gets \decrypt(c, \encpp, \sk)$. Compute $c_1^{-\sk} * c_2$ to get $g^m$, and then brute force\footnote{This is fine in blockchain applications because people usually know their own balance, and can always brute-force in a small range.} $m$. 
    \end{itemize}
    Note that other encryption schemes can also be used if they are additively homomorphic and statistically (or computationally) hiding.
\end{definition}
\fi

